The Grow-Shrink strategy for learning Markov network structures constrained by context-specific independences

Markov networks are models for compactly representing complex probability distributions. They are composed by a structure and a set of numerical weights. The structure qualitatively describes independences in the distribution, which can be exploited to factorize the distribution into a set of compact functions. A key application for learning structures from data is to automatically discover knowledge. In practice, structure learning algorithms focused on "knowledge discovery" present a limitation: they use a coarse-grained representation of the structure. As a result, this representation cannot describe context-specific independences. Very recently, an algorithm called CSPC was designed to overcome this limitation, but it has a high computational complexity. This work tries to mitigate this downside presenting CSGS, an algorithm that uses the Grow-Shrink strategy for reducing unnecessary computations. On an empirical evaluation, the structures learned by CSGS achieve competitive accuracies and lower computational complexity with respect to those obtained by CSPC.

==> alg-feature-generation.tex <==
% Feature Generation
\begin{algorithm}[!h]\small
  \KwIn{Canonical model \(\bar\G\)}

  \BlankLine

  \(\F \leftarrow\emptyset\)

  \ForEach {\(G(x^i)\in\bar\G\) }
  {
    \ForEach {maximum clique C \(\in G(x^i)\)}
    {
      \(\F \leftarrow \F \cup\{x^i_C\}\)
    }
  }

  \(\F \leftarrow\) Add unit feature \(x^i_a\) for each variable \(X_a\in X\)

  \Return{\F}

  \caption{\textsc{Feature Generation}}
  \label{alg:cspc:generation}
\end{algorithm}
